The Method of Conditional Expectations for Cubic Metric Reduction in OFDM

High variations in the OFDM signal envelope cause nonlinear distortion in the power amplifier of the transmitter, which is a major drawback. Peak-to-Average Power Ratio (PAPR) and Cubic Metric (CM) are commonly used for quantifying this characteristic of the signal. Despite the reportedly higher accuracy compared to PAPR, limited research has been done on reduction algorithms for CM. In this paper, the Method of Conditional Expectations (CE Method) is used to achieve CM reduction by the Sign Selection approach. Using the CE Method, the amenable mathematical structure of CM is exploited to develop a low complexity algorithm. In addition, guaranteed reduction is analytically proved for every combination of the data symbols. Simulations show a reduction gain of almost 3 dB in Raw Cubic Metric (RCM) for practically all subcarrier numbers, which is achieved using only half the full rate loss of the Sign Selection approach.

==> tikz-files/frame-double.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (13.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\foreach \x in {3,4,5}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\foreach \x in {6,7,8}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (9,1) rectangle +(0.5,-0.15);


\foreach \x in {6,7,8}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);

\foreach \x in {9,10,11}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);


\fill [draw=blue, fill=white, rounded corners=0.02cm] (12,1.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> tikz-files/frame-single.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (7.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \xone/\y in {0/0.8, 0.5/1, 1/1.3, 1.5/1.5, 2/1.8, 2.5/2}
{
	\draw [blue,|-|] (\xone,\y) -- +(4,0);
}

\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> tikz-files/pts-oqam-structure.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\usetikzlibrary{positioning}
%
%\input{ tikz-styles}
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}

%%%%%%%%the modulator

\node[block,minimum width=1.5cm] (filter1) {SFB};
\node[block,minimum width=1.5cm] (filter2) [below=of filter1, yshift=0.5cm] {SFB};
\node[block,minimum width=1.5cm] (filter3) [below=of filter2, yshift=0.5cm] {SFB};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (partitioning) [left of=filter1, xshift=-0.2cm, yshift=+2cm] {Partitioning};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (OQAMpre) [left of=filter1, xshift=-0.2cm, yshift=+3.8cm] {OQAM pre-preprocessing};

\node[block,minimum width=1cm, minimum height=3.7cm] (sum) [right of=filter2, xshift=4cm, yshift=0cm] {$\sum$};


\node (mul1) [summul, right of=filter1, xshift=1cm] {$\times$};
\node (mul2) [summul, right of=filter2, xshift=1.5cm] {$\times$};
\node (mul3) [summul, right of=filter3, xshift=2cm] {$\times$};

\draw [<-] (mul1) -- +(0,0.6cm) node [anchor=west]{$p_1$};
\draw [<-] (mul2) -- +(0,0.6cm) node [anchor=west]{$p_2$};
\draw [<-] (mul3) -- +(0,0.6cm) node [anchor=west]{$p_3$};

\foreach \x in {1,2,3}
	\draw [->] (filter\x) -- (mul\x);

\draw [->] (mul1.east) -- +(2.32cm,0);
\draw [->] (mul2.east) -- +(1.82cm,0);
\draw [->] (mul3.east) -- +(1.32cm,0);

\node[block,minimum width=2.4cm, minimum height=1cm] (opt) [below of=mul2, xshift=0cm, yshift=-2cm] {Optimization};

\draw [<-] (mul1) |- (opt.north);
\draw [<-] (mul2) -- (opt);
\draw [<-] (mul3) |- (opt.north);
%\draw [<-] (mul2) -- +(0cm,0);
%\draw [<-] (mul3) -- +(0cm,0);

%\foreach \x/\n in {1/0,2/1,3/N-1}
%	\draw [<-] (mul\x) -- +(0,0.5cm) node [anchor=south] {$\beta_{\n}$};

\foreach \x in {1,2,3}
{
	\draw [<-] (filter\x.west) -- +(-0.73cm,0) ;		%between SFB and partitioning
}

\draw [->] (filter1.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,0}$};  %between input and OQAM
\draw [->] (filter2.west) +(-4.5cm,0.5cm)-- +(-3.55cm,0.5cm) node [anchor=south east] {$A_{k,1}$};  %between input and OQAM
\draw [->] (filter3.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,N-1}$};  %between input and OQAM

\draw [->] (filter1.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	
\draw [->] (filter2.west) +(-2.55cm,0.5cm)-- +(-1.75cm,0.5cm) ;	%between OQAM and partitioning	
\draw [->] (filter3.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	

\node[circle, fill=black, left=of partitioning, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.3cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[circle, fill=black, left=of OQAMpre, yshift=1.9cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[block,minimum width=2cm, minimum height=1cm] (buffer) [above of=sum, xshift=-0.5cm, yshift=1.7cm] {Buffer};

\draw [->] (buffer.west) -- +(-0.3cm,0) -- +(-0.3cm,-1.2cm) -- +(1cm,-1.2cm);
\draw [->] (sum.east) +(1cm,0) |- (opt.east);
\draw [->] (sum.east) +(1cm,0) |- (buffer.east);
\draw [->] (sum.east) -- +(1.5cm,0) node [anchor=south] {$s[k]$};


	
\end{tikzpicture}
%\end{figure}
%\end{document}


==> version 7 submitted to SPAWC19 arxiv/tikz-files/frame-double.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (13.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\foreach \x in {3,4,5}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\foreach \x in {6,7,8}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (9,1) rectangle +(0.5,-0.15);


\foreach \x in {6,7,8}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);

\foreach \x in {9,10,11}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);


\fill [draw=blue, fill=white, rounded corners=0.02cm] (12,1.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> version 7 submitted to SPAWC19 arxiv/tikz-files/frame-single.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (7.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \xone/\y in {0/0.8, 0.5/1, 1/1.3, 1.5/1.5, 2/1.8, 2.5/2}
{
	\draw [blue,|-|] (\xone,\y) -- +(4,0);
}

\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> version 7 submitted to SPAWC19 arxiv/tikz-files/pts-oqam-structure.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\usetikzlibrary{positioning}
%
%\input{ tikz-styles}
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}

%%%%%%%%the modulator

\node[block,minimum width=1.5cm] (filter1) {SFB};
\node[block,minimum width=1.5cm] (filter2) [below=of filter1, yshift=0.5cm] {SFB};
\node[block,minimum width=1.5cm] (filter3) [below=of filter2, yshift=0.5cm] {SFB};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (partitioning) [left of=filter1, xshift=-0.2cm, yshift=+2cm] {Partitioning};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (OQAMpre) [left of=filter1, xshift=-0.2cm, yshift=+3.8cm] {OQAM pre-preprocessing};

\node[block,minimum width=1cm, minimum height=3.7cm] (sum) [right of=filter2, xshift=4cm, yshift=0cm] {$\sum$};


\node (mul1) [summul, right of=filter1, xshift=1cm] {$\times$};
\node (mul2) [summul, right of=filter2, xshift=1.5cm] {$\times$};
\node (mul3) [summul, right of=filter3, xshift=2cm] {$\times$};

\draw [<-] (mul1) -- +(0,0.6cm) node [anchor=west]{$p_1$};
\draw [<-] (mul2) -- +(0,0.6cm) node [anchor=west]{$p_2$};
\draw [<-] (mul3) -- +(0,0.6cm) node [anchor=west]{$p_3$};

\foreach \x in {1,2,3}
	\draw [->] (filter\x) -- (mul\x);

\draw [->] (mul1.east) -- +(2.32cm,0);
\draw [->] (mul2.east) -- +(1.82cm,0);
\draw [->] (mul3.east) -- +(1.32cm,0);

\node[block,minimum width=2.4cm, minimum height=1cm] (opt) [below of=mul2, xshift=0cm, yshift=-2cm] {Optimization};

\draw [<-] (mul1) |- (opt.north);
\draw [<-] (mul2) -- (opt);
\draw [<-] (mul3) |- (opt.north);
%\draw [<-] (mul2) -- +(0cm,0);
%\draw [<-] (mul3) -- +(0cm,0);

%\foreach \x/\n in {1/0,2/1,3/N-1}
%	\draw [<-] (mul\x) -- +(0,0.5cm) node [anchor=south] {$\beta_{\n}$};

\foreach \x in {1,2,3}
{
	\draw [<-] (filter\x.west) -- +(-0.73cm,0) ;		%between SFB and partitioning
}

\draw [->] (filter1.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,0}$};  %between input and OQAM
\draw [->] (filter2.west) +(-4.5cm,0.5cm)-- +(-3.55cm,0.5cm) node [anchor=south east] {$A_{k,1}$};  %between input and OQAM
\draw [->] (filter3.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,N-1}$};  %between input and OQAM

\draw [->] (filter1.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	
\draw [->] (filter2.west) +(-2.55cm,0.5cm)-- +(-1.75cm,0.5cm) ;	%between OQAM and partitioning	
\draw [->] (filter3.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	

\node[circle, fill=black, left=of partitioning, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.3cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[circle, fill=black, left=of OQAMpre, yshift=1.9cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[block,minimum width=2cm, minimum height=1cm] (buffer) [above of=sum, xshift=-0.5cm, yshift=1.7cm] {Buffer};

\draw [->] (buffer.west) -- +(-0.3cm,0) -- +(-0.3cm,-1.2cm) -- +(1cm,-1.2cm);
\draw [->] (sum.east) +(1cm,0) |- (opt.east);
\draw [->] (sum.east) +(1cm,0) |- (buffer.east);
\draw [->] (sum.east) -- +(1.5cm,0) node [anchor=south] {$s[k]$};


	
\end{tikzpicture}
%\end{figure}
%\end{document}


==> version 7 submitted to SPAWC19 arxiv/tikz-files/tikz-styles.tex <==
\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\tikzstyle{axis-line}=[thick, ->, >=stealth]
\tikzstyle{axis-tick}=[thin]
\tikzstyle{arrow} = [thick,->]

\tikzstyle{block}=[rectangle,black,draw, text centered, minimum height=0.7cm]
\tikzstyle{summul} = [draw, shape=circle, text centered,inner sep=0]




